Canonical Capsules: Self-Supervised Capsules in Canonical Pose

We propose a self-supervised capsule architecture for 3D point clouds. We compute capsule decompositions of objects through permutation-equivariant attention, and self-supervise the process by training with pairs of randomly rotated objects. Our key idea is to aggregate the attention masks into semantic keypoints, and use these to supervise a decomposition that satisfies the capsule invariance/equivariance properties. This not only enables the training of a semantically consistent decomposition, but also allows us to learn a canonicalization operation that enables object-centric reasoning. To train our neural network we require neither classification labels nor manually-aligned training datasets. Yet, by learning an object-centric representation in a self-supervised manner, our method outperforms the state-of-the-art on 3D point cloud reconstruction, canonicalization, and unsupervised classification.

==> fig/teaser.tex <==

\begin{wrapfigure}{R}{0.5\linewidth}
\vspace{-20pt}
\begin{center}
    \begin{overpic}
        [width=\linewidth]
        {fig/teaser.png}
    \end{overpic}
    \vspace{-.5em}
    \caption{
        \TODO{Maybe delete it for space. Remember mention mental picture somewhere.}
        \textbf{Teaser -- }
        We design a capsule architecture $\acne$ that is trained in an unsupervised fashion -- by only observing \textit{pairs} of randomly rotated 3D point clouds (of the \textit{same} object).
        The architecture builds a $K$-fold decomposition that estimates primary capsules whose descriptors are \textit{invariant} to rigid transformations, and whose poses -- i.e.~keypoints that summarize the location of a part -- are transformation \textit{equivariant}.
        By relating capsule poses to capsule descriptors, the network $\regressor$ introduces the concept of a ``mental picture'' of an object: an object-centric coordinate frame for the object that empowers downstream tasks such as auto-encoding and classification.
    }
    \label{fig:teaser}
    \end{center}
\vspace{-20pt}
\vspace{1pt}
\end{wrapfigure}

\endinput


